Riemannian Residual Neural Networks

Recent methods in geometric deep learning have introduced various neural networks to operate over data that lie on Riemannian manifolds. Such networks are often necessary to learn well over graphs with a hierarchical structure or to learn over manifold-valued data encountered in the natural sciences. These networks are often inspired by and directly generalize standard Euclidean neural networks. However, extending Euclidean networks is difficult and has only been done for a select few manifolds. In this work, we examine the residual neural network (ResNet) and show how to extend this construction to general Riemannian manifolds in a geometrically principled manner. Originally introduced to help solve the vanishing gradient problem, ResNets have become ubiquitous in machine learning due to their beneficial learning properties, excellent empirical results, and easy-to-incorporate nature when building varied neural networks. We find that our Riemannian ResNets mirror these desirable properties: when compared to existing manifold neural networks designed to learn over hyperbolic space and the manifold of symmetric positive definite matrices, we outperform both kinds of networks in terms of relevant testing metrics and training dynamics.

==> figures/afew.tex <==
\begin{table*}[h]
\centering
%\addtolength{\tabcolsep}{2pt}
\begin{tabular}{c|rrr}
\hline
 & Val Accuracy & No. of Parameters \\ 
\hline
SPDNet \citep{Huang2017ARN} && 37507\\
SPDNetBN \citep{Brooks2019RiemannianBN} && 40007\\
RResNet with Spectrum Map (Ours) && 42577\\

\hline

\end{tabular}
\caption{Results and standard deviations are averaged over five trials.}
\label{tab:afew}
\end{table*}

==> figures/afew_graph.tex <==
\begin{wrapfigure}{R}{.4\textwidth}
    \vspace{-10pt}
%\includegraphics[width=0.4\textwidth]{figures/AFEW.pdf}
%\includegraphics[width=0.4\textwidth]{figures/FPHA.pdf}
\includegraphics[width=0.4\textwidth]{figures/HDM05.pdf}
%\includegraphics[width=0.4\textwidth]{figures/NTURGBD.pdf}

\caption{ We observe that our model converges faster and achieves higher accuracies than SPDNet and SPDNetBN.}
\label{fig:afew_graph}
\vspace{-15pt}
\end{wrapfigure}

==> figures/hyperbolic_old.tex <==
\begin{table*}[h]
\centering
\scalebox{1.0}{
\begin{tabular}{ccccc}
\hline
\textbf{Dataset}       & \multicolumn{2}{c}{Airport}      & \multicolumn{2}{c}{PubMed}         \\
\textbf{Hyperbolicity} & \multicolumn{2}{c}{$\delta = 1$} & \multicolumn{2}{c}{$\delta = 3.5$} \\ \cline{2-5} 
\textbf{Task}          & LP    & \multicolumn{1}{c}{NC}   & LP\footnotemark     & \multicolumn{1}{c}{NC}    \\ \hline
HNN     & \multicolumn{1}{c}{$93.0$\tiny$\pm 0.8$}          & $60.9$\tiny$\pm 0.4$          & \hspace{0.25in}$94.9$\tiny$\pm 0.1$ \hspace{0.25in} & $69.6$\tiny$\pm 1.0$          \\
RResNet & \multicolumn{1}{c}{$\mathbf{95.1 \pm 0.1}$} & $\mathbf{72.4 \pm 2.4}$ & \hspace{0.25in}--\hspace{0.25in} & $\mathbf{72.5 \pm 1.0}$ \\ \hline
\end{tabular}}
\caption{The metrics reported are ROC AUC for link prediction (LP) and F1-score for node classification (NC). Ten trials were conducted; mean and standard deviation are reported. We compare the performance of HNN, as implemented by \citet{chami2019hyperbolic}, to RResNet. Note that we considerably outperform the baseline while using fewer parameters. The best result on each task is bolded.}
\label{tab:hyperbolichnn}
\end{table*}
\footnotetext{We had numerical issues with LP on PubMed that prevented us from obtaining stable results across trials.}
